Using Recurrent Neural Network for Learning Expressive Ontologies

Recently, Neural Networks have been proven extremely effective in many natural language processing tasks such as sentiment analysis, question answering, or machine translation. Aiming to exploit such advantages in the Ontology Learning process, in this technical report we present a detailed description of a Recurrent Neural Network based system to be used to pursue such goal.

==> assesment.tex <==
\section{First Assessment}
\label{sec:assessment}

We tested the feasibility of our approach with an experiment. In this section we will also describe the language model we used as a source language and the description logic constructs we took in consideration for the target language. We will describe the network architectures in the concrete case through its hyperparameters and show the results of our experiment.

% definition of source and target language
\subsection{Source and Target Languages.}
\label{sec:assessment-sourcetargetlang}

To the best of our knowledge, there is no commonly accepted benchmark for the ontology learning task, so we had to build our own test bench. 
In our first assessment, as in \cite{grefenstette2015learning, zaremba2014learning, weston2014memory, peng2015towards}, we restricted the expressiveness of our source language to definition-like sentences, as typically found in encyclopedias, like~\eqref{eq:sentence}.
We verbalized all the possible OWL constructs and their combinations in order to generate a start set of definitory sentences, then manually extended such set adding some variations of every verbalization.
Finally, we build a grammar capable to generate all such sentences, with placeholders instead 
of \emph{concepts}, \emph{roles}, and numbers used in cardinality restriction clauses. 
All the definitions have a left hand side class description which subsumes a right hand side description. Each side can be itself made of one or two \emph{atomic} definitions, conjuncted or disjuncted, which can be \emph{concepts} definition or \emph{roles} definitions. 
Roles can be bound to one or two cardinality constraints, conjuncted or disjuncted. 
At the same time, we restricted the target language to a subset of the $\mathcal{SHOIN^{(D)}}$ description logic -- which \texttt{OWL-DL} is based on -- made of: concepts, roles, subsumption, concept intersection and union, existential restriction, cardinality restrictions maybe in conjunction or disjunction.
From our grammar, we generated 786 different \emph{sentence templates}; we manually annotated them obtaining 127 different formula templates, built using the constructs listed right before. Some examples of sentences and corresponding formulae are in Table~\ref{tab:examples}.
%
\begin{table}[tbh]
\caption{Examples of sentence templates and formula templates}
\centering
{\scriptsize
  \begin{tabular}[c]{c | c}
    \hline
    \centering \textbf{sentence template} & \centering \textbf{formula template} \tabularnewline
    \hline \hline
    \textit{anything that} $\mathtt{R_0}$ \textit{at least} $\mathtt{N_0}$ $\mathtt{C_0}$ \textit{and is also} $\mathtt{C_1}$ \textit{, is} $\mathtt{C_2}$ & 
    $\geqslant \mathtt{N_0} \mathtt{R_0}.\mathtt{C_0} \sqcap \mathtt{C_1} \sqsubseteq \mathtt{C_2}$ \\ \hline
    \textit{every} $\mathtt{C_0}$ \textit{is also something that} $\mathtt{R_0}$ \textit{less than} $\mathtt{N_0}$ \textit{or more than} $\mathtt{N_1}$ $\mathtt{C_1}$ & 
    $\mathtt{C_0} \sqsubseteq < \mathtt{N_0} \mathtt{R_0}.\mathtt{C_1} \sqcup > \mathtt{N_1} \mathtt{R_0}.\mathtt{C_1}$ \\ \hline
    \textit{anything that} $\mathtt{R_0}$ \textit{less than} $\mathtt{N_0}$ \textit{or more than} $\mathtt{N_1}$ $\mathtt{C_0}$ \textit{is} $\mathtt{C_1}$ & 
    $< \mathtt{N_0} \mathtt{R_0}.\mathtt{C_0} \sqcup > \mathtt{N_1} \mathtt{R_0}.\mathtt{C_0} \sqsubseteq > \mathtt{C_1}$ \\ \hline
  \end{tabular}
}
\vspace{1em}

\label{tab:examples}
\end{table}
%
\subsection{Training and Test Set}
To turn a sentence template into an actual sentence, we have to fill its placeholder with actual words. 
\emph{Role} placeholders are filled with verbs, randomly selected from a list of 840. Each \emph{concept} placeholder is filled combining words from a list of 36 adjectives, a first list of 50 nouns and a second list of 92 nouns. Combinations were allowed only according to the patterns presented in Tab.\ref{tab:conc-patterns}. 

\begin{table}[tbh]
  \caption{Patterns for concept name generation}
  \centering
  \begin{tabular}[c]{c|c|c}
    \hline
    \textbf{adjective} & \textbf{noun\#1} & \textbf{noun\#2} \\
    \hline \hline
    magnificent & sword & sharpener \\
    \st{ }  &  sword & sharpener \\
    magnificent & \st{ } &  sharpener \\
    magnificent & sword & \st{ } \\
    \st{ } & sword & \st{ } \\
     \st{ } & \st{ } & sharpener \\
  \end{tabular}
  \vspace{1em}
  \label{tab:conc-patterns}
\end{table}

We ended up in 185706 possible combinations. Numbers, used only in cardinality restrictions, are treated in a different way, as the placeholders are not filled with actual numbers. This missing substitution can be seen as the only text pre-processing phase for number identification, which is a task that can be performed easily with a rule based approach. As an example, see Tab.\ref{tab:patterntoex}.
%
\begin{table}[tbh]
  \caption{From a pattern to an example.}
  \centering
  \begin{tabular}[]{r|c}
    \hline
    \textbf{sentence template} & \textit{A} $\mathtt{C_0}$ \textit{is a} $\mathtt{C_1}$ \textit{that} $\mathtt{R_0}$ \textit{exactly} $\mathtt{N_0}$ $\mathtt{C_2}$ \\ \hline \hline
    \textbf{sentence} & \textit{A bee is a insect that has exactly}  $\mathtt{N_{0}}$ \textit{legs} \\
    \textbf{tag set} & \texttt{w} $\mathtt{C_0}$ \texttt{w} \texttt{w} $\mathtt{C_1}$ \texttt{w} $\mathtt{R_0}$ \texttt{w} $\mathtt{N_0}$ $\mathtt{C_2}$ \\
    \textbf{formula template} & $\mathtt{C_0} \sqsubseteq \mathtt{C_1} \sqcap = \mathtt{N_{0}} \mathtt{R_0.C_2}$ \\
  \end{tabular}
  \vspace{1em}
  \label{tab:patterntoex}
\end{table}

We built our training set generating 10 examples for each sentence template, ending up in 7860 examples. We ended up in a vocabulary of 1044 words, 10 tags and 18 formula terms. Once generated the training set, we generated a test set in order to evaluate the system after the training phase. We used the same vocabulary of the training set. W.r.t. the test set, we want to remark that, even if using the same words for \emph{concept} used in the training set, it could be the case that new combination of the same words are used. So, if we found \emph{``awesome gate controller''} and \emph{``empty head''} filling some \emph{concept}  placeholder, we could end up having \emph{``awesome head''} in the test set, even if this combination doesn't appear in the training set. Generating the test set, we ensured that no actual sentence in the test set is in the training set, so there is no chance for our system to just memorize the examples. All the sentence will be grammatically correct, even if unrealistic from a human point of view -- e.g. \emph{``A massive analyzer is also something that fit at least 13 orange stampede''}.

\subsection{Experimental Setting and Results.}
For both the tasks, we defined the network dimension empirically, according to some experiences in literature. 
We trained both the networks with AdaDelta (see \cite{zeiler2012adadelta}) for 150 epochs. The network configurations, together with the training parameters, are reported synthetically in Fig.~\ref{fig:params}. At each epoch, randomly split the dataset in 90\% for training and 10\% of validation, ensuring the same ratio for all the sentences stemmed from the same sentence template. We used the categorical cross entropy as the cost function. As expected, the validation accuracy reached 100\% after few epochs, as shown in Fig.~\ref{fig:validacc} -- only the first 10 and 50 epochs are reported for sentence tagging and sentence transduction respectively. We tested the trained newtorks on the test set, obtaining, as expected, 100\% of classification accuracy as well.

\begin{figure}[tbh]
  \begin{minipage}[b]{0.5\textwidth}
    \centering
    \input{validationaccuracy-tikz}
    \caption{Validation accuracy}
    \label{fig:validacc}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4\textwidth}
    \scriptsize
    \centering
   \begin{tabular}[t]{c|c}
     \multicolumn{2}{c}{\textbf{Sentence Tagging}}\\
     \hline
     $\left\vert V_{in} \right\vert$ & 1044 \\
     dim. embedding & 100 \\
     dim. hidden & 200 \\
     $\left\vert V_{out} \right\vert$ & 10 \\
     \multicolumn{2}{c}{}\\
     
     \multicolumn{2}{c}{\textbf{Sentence Transduction}}\\
     \hline
     $\left\vert V_{in} \right\vert$ & 1044 \\
     dim. embedding & 100 \\
     dim. encoding & 1000 \\
     dim. decoding & 1000 \\
     $\left\vert V_{out} \right\vert$ & 17 \\
     \multicolumn{2}{c}{}  \\
     
     \multicolumn{2}{c}{\textbf{Training parameters}}\\
     \hline
     epochs & 150 \\
     batch size & 128 \\
     learning rate & 2.0 \\
     $\rho$ & 0.95 \\
     $\epsilon$ & $10^{-6}$ \\
   \end{tabular}
   \caption{Network parameters}
   \label{fig:params}
  \end{minipage}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We generated a second test set $\mathcal{T}_A$ using a lexicon compliant with the Attempto Parser Engine (APE).\footnote{\url{http://attempto.ifi.uzh.ch/site/resources/}} 
The APE engine could parse only 80 sentences from 786 and among them only 20 where correctly parsed. 
A qualitative analysis through the sentences not or incorrectly parsed by the APE service gave us an idea of all the linguistic phenomena that our system can handle beyond the controlled language. We can roughly split them in two groups:

\begin{enumerate}
  \item function words that are not parsed by the controlled language but that are actually used in natural language, such as:
    \begin{enumerate}
    \item \emph{``anything''} as a universal quantifier
    \item \emph{``at least''} or \emph{``exactly''} for cardinality restriction
    \item \emph{``also''}, in the right hand side of an implication, e.g. \emph{``if something is a mammal, it is also an animal''}
    \end{enumerate}

\item constructs that are not parsed by the controlled language but are actually used in natural language, such as: 
\begin{enumerate}
\item ellipsis of the demonstrative pronoun \emph{``that''} in conjunction or disjunctions, e.g. \emph{``everything that barks and (that) chases cats, is a dog''}
\item ellipsis of the demonstrative pronoun, role and range concept in conjunction or disjunction of cardinality restrictions, e.g. \emph{``a bass is an instruments that has at least 4 (strings) or (that has) at most 6 strings''}
\item ellipsis of the adverb in cardinality restriction, instead of \emph{``exactly''}, as in \emph{``a bee is an insect that has (exactly) 6 legs''}
\item ellipsis of the quantifier, as in \emph{``dogs are mammals''}
\item \emph{``everything that is''} as a quantifier
\end{enumerate}
\end{enumerate}

The language model we built actually covers just a small fractions of the formalization that can be modeled with a controlled language like Attempto, but such analysis already gives us some hints about the effectiveness of our approach as, on the long term, more phenomena could be learned with an reduced effort.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:


==> ontolearnasmt.tex <==
%!TEX root = ./master.tex

\section{Ontology Learning as a Transduction task}
\label{sec:ontolearnasmt}

The main intuition underpinning our approach is that ontology learning can be seen as a \emph{transduction} process, as defined in \cite{grefenstette2015learning}: a string from a source language is converted into another string of a target language. In our specific case, we want to convert a sequence of words, that is a \emph{sentence} in natural language, into a sequence of logical symbols, namely a \emph{formula}. As an example, let us consider the following sentence: 
%
\begin{quotequation}
  \centering
  \emph{``A bee is an insect that has 6 legs and produces honey.''} 
  \label{eq:sentence}
\end{quotequation}
%
This sentence provides a brief description of a bee and of its main characteristics and can be encoded by means of the following DL formula which, so-to-speak, represents the conversion of \eqref{eq:sentence} into a formula: 
\begin{equation}
  \label{eq:definition}
  \mathtt{Bee} \sqsubseteq \mathtt{Insect} \sqcap =\mathtt{6} \ \mathtt{have}.\mathtt{Leg} \sqcap \exists \mathtt{produce}.\mathtt{Honey}
\end{equation}
Nouns like \texttt{Bee}, \texttt{Insect}, \texttt{Leg} and \texttt{Honey} denote the involved \emph{concepts} while verbs like \texttt{have} and \texttt{produce} describe relationships  among such concepts, or \emph{roles}. From a linguistic standpoint, nouns and verbs -- together with adjectives and some adverbs -- are \emph{content words} as they describe the actual content of a sentence. Dually, words such as articles, pronouns, conjunctions, most adverbs, etc. are considered \emph{function words} as they express grammatical relationships between words and carry almost no lexical meaning. 

One of the problems we have in converting natural language sentences into logical formulae is the variability of natural language. Consider for instance:
%
\begin{quotequation}
  \label{eq:altsentence}
  \centering
  \emph{``If something is a bee, then it is an insect \\ with exactly 6 legs and it also produces honey.''}
\end{quotequation}
Despite being lexically and syntactically different from \eqref{eq:sentence}, \eqref{eq:altsentence} provides a description of a bee which is, from the standpoint of an ontological formulation, equivalent to the one provided in \eqref{eq:sentence}. Thus, we would like to be able to transform it into the same formula \eqref{eq:definition}. 
We can also notice that content words are \emph{the same} across sentences \eqref{eq:sentence} and \eqref{eq:altsentence}, while function words changes. 

A second, dual, problem we have in converting natural language sentences into logical formulae is the fact that sentences often ``share'' a similar structure while conveying a completely different meaning. An exemplification of this problem is provided by the sentence:
\begin{quotequation}
  \label{eq:diffsentence}
  \centering
  \emph{``A cow is a mammal that has 2 horns and eats grass''}
\end{quotequation}
%
which shares several similarities with sentence \eqref{eq:sentence}, and would be translated into a DL formula such as 
\begin{equation}
  \label{eq:diffdefinition}
  \mathtt{Cow} \sqsubseteq \mathtt{Mammal} \sqcap =\mathtt{2} \ \mathtt{have}.\mathtt{Horns} \sqcap \exists \mathtt{eat}.\mathtt{Grass}
\end{equation}
which is, from a structural point of view, very similar to the one in \eqref{eq:definition}.
In this case we can note that sentence \eqref{eq:diffsentence} shares the same function words of \eqref{eq:sentence}, while content words are radically different. 

\begin{figure}[t]
  \centering
  \input{pipeline-tikz.tex}
  \caption{The whole pipeline}
  \label{fig:pipeline}
\end{figure}
Our idea is to deal with these two problems by splitting the transduction process of sentences such as \eqref{eq:sentence}, \eqref{eq:altsentence}, and \eqref{eq:diffsentence} in two parallel phases: a \emph{sentence transduction} phase and a \emph{sentence tagging} phase as depicted in Figure \ref{fig:pipeline}. The sentence transduction phase focuses on the identification of the logical structure of the formula corresponding to the natural language specification. The output of this phase is a structure that we name \emph{formula template}. For sentences \eqref{eq:sentence}, \eqref{eq:altsentence}, and \eqref{eq:diffsentence} the formula template is:
\begin{equation}
  \label{eq:formula}
  \mathtt{C_0} \sqsubseteq \mathtt{C_1} \sqcap =\mathtt{N_0} \ \mathtt{R_0}.\mathtt{C_2} \sqcap \exists \mathtt{R_1}.\mathtt{C_3}
\end{equation}
where \texttt{C}, \texttt{R} and \texttt{N} have been respectively used for concepts, roles and numbers, with a subscripts indicating their order. Sentence transduction is therefore the phase which tackles the challenge of identifying a common unifying structure among different natural language sentences that may differ both lexically and syntactically.

The sentence tagging phase focuses on identifying and recognising all the content words for what they act in the sentence: concept, role, number or generic word. The output of this phase for the three sentences is: 
\begin{align}
  \label{eq:taggedseq}
  \begin{split}
  A \  & [bee]_{\mathtt{C_0}} \ is \ an \ [insect]_{\mathtt{C_1}} \ that \ [has]_{\mathtt{R_0}}
   [6]_{\mathtt{N_0}} \ [legs]_{\mathtt{C_2}} \ and \\ & [produces]_{\mathtt{R_1}} \ [honey]_{\mathtt{C_3}}
  \end{split}\\[0.5ex]
  \label{eq:taggedalternateseq}
  \begin{split}
     If & \ something  \ is \ a \ [bee]_{\mathtt{C_0}} \ is \ an \ [insect]_{\mathtt{C_1}} \ that \ [has]_{\mathtt{R_0}} \ exactly \\
    & [6]_{\mathtt{N_0}}  \ [legs]_{\mathtt{C_2}} \ and \ it \ also \ [produces]_{\mathtt{R_1}} \ [honey]_{\mathtt{C_3}}
  \end{split}\\[0.5ex]
  \label{eq:taggeddiffseq}
  \begin{split}
    A & \ [cow]_{\mathtt{C_0}} \ is \ a \ [mammal]_{\mathtt{C_1}} \ that [has]_{\mathtt{R_0}} \ [4]_{\mathtt{N_0}} \ [legs]_{\mathtt{C_2}}  and \\ & [eats]_{\mathtt{R_1}} \ [grass]_{\mathtt{C_3}}
  \end{split}
\end{align}

where all the words other than \texttt{C}, \texttt{R}, or \texttt{N} are intended to be tagged with a generic word label, \texttt{w}. This step is close to the slot filling problem, as tackled in \cite{mesnil2013investigation}: we need to detect the role each word assumes within a certain semantic scope, even a whole sentence. 

The final step in the pipeline is to combine the outputs of the two phases to obtain the resulting logical formula. Thus, the formula template  \eqref{eq:formula} combined with the tagged sentences \eqref{eq:taggedseq} and \eqref{eq:taggedalternateseq} will provide formula \eqref{eq:definition} as the logical conversion for both sentences \eqref{eq:sentence} and \eqref{eq:altsentence}, while the formula template  \eqref{eq:formula} combined with the tagged sentence \eqref{eq:taggeddiffseq} will provide formula \eqref{eq:diffdefinition} as the logical conversion of sentence \eqref{eq:diffsentence}. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:

==> stateoftheart.tex <==
\section{State of the Art}
\label{sec:soa}

In this section, we will present a short overview on those ontology
learning approaches focused on the extraction of expressive
knowledge. For a wider description of the state of the art in such
field, see \cite{cimiano2009ontologylearning,petrucci2015information}
Next, we will recap some recent works in the field of neural networks
in the field of natural language that exploits deep neural network
architectures.


\subsection{Ontology Learning}
\label{sec:soa-ontolearn}

Since OWL emerged as the \emph{de facto} ontology language standard
for the Semantic Web, many effort has been put in the direction of
fully exploit its expressive capabilities. From the ontology learning
standpoint, many significant results have been achieved: tasks
taxonomy construction and factual knowledge extraction -- assertions,
entities, relation -- can be fully automatized with good
performance. But despite such progress, quoting authors of
\cite{volker2008lexo}, state of the art methods are \emph{able to
  generate ontologies that are largely informal}, that is
\emph{limited in their expressiveness}.

$\mathcal{EL}$\verb!++! definition can be extracted by text fragments
involving concepts from the \textsc{Snomed
  CT}\footnote{\url{http://www.ihtsdo.org/snomed-ct/}} ontology using a
maximum entropy classifier, as shown in \cite{ma2014hybrid}. Moreover
user feedback can be used to adaptively re-train the underlying model.

FRED (see \cite{presutti2012knowledgeextraction}) exploits Discourse
Representation Theory (DRT, see \cite{kamp1993drt}), a formal semantic
theory capable to handle contextually sensitive linguistic phenomena
such as anahporas, ellipsis, verb tense, etc. DRT represents text into
an explicit semantic representation called Discourse Representation
Structures (DRS), proven to be equivalent to First Order Logics (FOL),
which is evaluated by the Boxer parser (see \cite{bos2008boxer}). A
catalog of translation rules are then applied to transform such
representation into OWL constructs, relying on several external
linguistic
(FrameNet\footnote{\url{https://framenet.icsi.berkeley.edu/fndrupal/}},
VerbNet\footnote{\url{http://verbs.colorado.edu/~mpalmer/projects/verbnet.html}})
and ontological (FOAF,\footnote{\url{http://www.foaf-project.org/}}
DBpedia,\footnote{\url{http://http://dbpedia.org}} Dolce+DnS
Ultralite\footnote{\url{http://www.ontologydesignpatterns.org/ont/dul/DUL.owl}})
resources. Finally, a set of high level constraints called
\emph{Ontology Design Patterns} (ODPs) ensures a certain degree of
quality for the resulting ontolgies.

LExO (see \cite{volker2007acquisition}) uses a catalog of hand-crafted
syntactical rules applied to syntactic dependencies parse tree to turn
them into OWL axioms.  Such approach is the cornerstone of a wider
methodology presented in \cite{volker2008lexo} with the ambitious goal
to cover the whole ontology life-cycle management. In particular,
\emph{taxonomy overlap} of two detected concepts is used as a signal
to decide about their disjointness, through a ML based approach: the
less is likely that an instance of both the concepts exist in the
ontology, the more two classes are likely to be disjoint. Authors use
the WordNet\footnote{\url{https://wordnet.princeton.edu/}} taxonomy,
the similarity between the lexical context of the surface instances of
the concepts, some estimation of their Pointwise Mutual Information
(PMI) and a set of predefined lexico-syntactic patterns. 

State-of-the-art methods for a deeper knowledge extraction still
experience severe limitations.  Those working in a
sentence-by-sentence translation fashion are not able to handle
portions of knowledge that can be spread across different sentences.
Catalog of lexico-syntactic patterns are \emph{rigid} w.r.t. the
grammatical structure of the text they can process -- several
linguistic phenomena such as conjunctions, negations, disjunctions,
quantifiers scope, ellipsis, anaphora, etc., can be particularly hard
to parse and interpret. In addition, extending such catalog can be a
highly expensive task, as every single variation of every linguistic
phoenomenon must be explicitly encoded into a rule.  Finally, if bound
to a specific domain, they cannot generalize across different ones.


\subsection{Advances in Neural Networks for NLP}
\label{sec:soa-advancesnn}

% From NNs to Deep Learning
Neural networks are a well known family of statistical learning models which have been largely exploited for problems of classification, regression and clustering. 
Along the years, they have been employed in different areas: image processing, time series analysis, digital signal processing and natural language processing.
A well known problem in training multi-layered networks in gradient-based methods and backpropagation is the \emph{vanishing gradient} problem, first demonstrated in \cite{hochreiter1991untersuchungen}: a smaller and smaller fraction of the error is backpropagated back through these layers, significantly slowing down the training process.
Recently, the widespread of the GPU computing architectures provided researchers with a significantly increased amount of computing power, allowing to overcome such problem -- even if only in a pragmatical way, as remarked in \cite{schmidhuber2014dl}.
In this scenario, a new interest flourished in \emph{deep} network architectures, which were already theoretically established and proved to be advantageous (see \cite{bengio2009learning}).
As a consequence, different complex network architectures exploiting different neural cell models, have been used for several tasks achieving remarkable results.
A sort of new discipline arisen, commonly referred to as \emph{deep learning}, aiming to exploit such systems to reduce the gap between Machine Learning and classical AI.

% Distribution representation of text
The main feature of these systems is that they can easily deal with distributed representations of text, which are extremely flexible and robust. 
Moreover, the dimensions of distributed vector space models are typically smaller of vocabulary dimensions, helping to avoiding the \emph{curse of dimensionality}.
Deep networks have been used to build a distributed representations of single words and to train a language model in the seminal work \cite{bengio2003neural}.
In \cite{collobert2011nlp} a single network architecture is trained to perform several typical NLP tasks: part-of-speech tagging, chunking, named entity recognition and semantic role labeling.
The main advantage of a unified learning process is that it is less dependent on intermediate representations or task-specific features: this ends up in a significant reduction of feature engineering costs.
In such approach, the distributed representation of words are learned from large amount of unlabeled training data.

% Recursive Neural Networks (RecNNs)
In Recursive Neural Networks (RecNNs, see \cite{goller1996learning}) two input vectors from a sequence are combined into a single vector of the same dimension, which is itself recursively combined with another vector from the input space: as long as we go through the recursion, the resulting vector will hold the distributed representation of larger and larger chuncks of text.
Such architectures have been successfully used to parse Natural Language sentences, as in \cite{socher2011parsing}, or for Sentiment Analysis, as in \cite{socher2013recursive}.
In \cite{bowman2015recursive}, RecNNs has also been used to evaluate a distributed representation of sentences for a task of Recognizing Textual Entailment (RTE) at the sentence level.

% Recurrent Neural Networks (RNNs)
Recurrent Neural Networks (RNNs) are fed sequentially: at each step, their state depends on the current input value and on their state at the previous step. This aspect makes them particularly suitable to model natural language sentences as a sequence of words. A pivotal aspect of such architecture is that, as long as we keep feeding it, we obtain a distributed representation that goes beyond the single word.
The usage of RNN architectures in the slot filling task has been explored in \cite{mesnil2013investigation}, with a minimum memory effect through windowing the input sequence. 
The network is endowed with a sort of memory effect by feeding it with juxtaposition of distributed vectors of single words as context windows of the central one.
Long Short-Term Memory (LSTM) units (see \cite{hochreiter1997long}) in order to achieve more powerful memory capabilities, are used in \cite{zaremba2014learning} where a RNN is trained to execute short fragment of python code in a sequence-to-sequence translation fashion.
In \cite{cho2014learning}, Gated Recursive Units (GRUs) are used for a machine translation task. Such units are conceptually simpler and computationally less expensive than LSTM ones, providing though a shorter term memory. In this approach, two RNNs are combined. The first one encodes the input sequence into a single vector. Such vector is then fed into the second RNN which acts as a decoder, generating the output sequence.
A more complex architecture of stacked GRU based RNNs is used in \cite{peng2015towards} for a task of question answering over the datasets presented in \cite{weston2015towards}: given some supporting facts and a question expressed in natural language, the system is trained to \emph{reason} about those facts in order to answer correctly.

% Long term memory enabled networks
Other approaches have tried to provide deep neural network with long term memory effect.
In \cite{weston2014memory} the associative memory it is provided with, allows the network to implement some sort of reasoning capabilities in a question-answering task over the datasets presented in \cite{weston2015towards}.
In \cite{grefenstette2015learning}, the network memory is built on the neural implementation of traditional data structures as Stacks, Queues and Double-Ended Queues. Such network is trained for a generic language transduction problem.

% Convolutional Neural Networks (CNNs)
Convolutional Neural Networks (CNNs) are feed-forward architectures that exploit local connectivity patterns: incoming connections for a hidden unit comes from other units of the previous layer which are \emph{similar} w.r.t. the features they describe. Such networks are trained in \cite{hermann2013multilingual} to learn distributed representations of sentences in different language without word alignment: the more two sentences from different languages have a similar distributed representation, the more are likely to have the same meaning. Such distributed representation can be seen as a sort of representation in a common, subsymbolic language.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:


==> taggingaccuracy.tex <==
epoch	accuracy
0	0.9945161007
1	0.9994296745
2	1
3	1
4	1
5	1
6	1
7	1
8	1
9	1
10	1


==> transductionaccuracy.tex <==
epoch	accuracy
0	0.441952926209
1	0.441952926209
2	0.441952926209
3	0.441952926209
4	0.449904580153
5	0.489662849873
6	0.489662849873
7	0.492048346056
8	0.465012722646
9	0.498727735369
10	0.521708015267
11	0.498489185751
12	0.494831424936
13	0.510337150127
14	0.533237913486
15	0.529739185751
16	0.595737913486
17	0.578005725191
18	0.583174300254
19	0.669529262087
20	0.679866412214
21	0.757872137405
22	0.740378498728
23	0.787770356234
24	0.787770356234
25	0.892493638677
26	0.903944020356
27	0.910702926209
28	0.937579516539
29	0.957617684478
30	0.993082061069
31	0.996421755725
32	0.999522900763
33	0.999920483461
34	1.0
35	1.0
36	1.0
37	1.0
38	1.0
39	1.0
40	1.0
41	1.0
42	1.0
43	1.0
44	1.0
45	1.0
46	1.0
47	1.0
48	1.0
49	1.0

%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: "master"
%%% End:


==> validationaccuracy-tikz.tex <==
\begin{tikzpicture}[scale=0.73]
\begin{axis}[
  xlabel=Epoch,
  ylabel=Accuracy,
  legend pos=south east
]
\addplot table [x=epoch, y=accuracy, col sep=tab, mark=''] {taggingaccuracy.tex};
\addlegendentry{{\scriptsize Sentence Tagging}};
\addplot table [x=epoch, y=accuracy, col sep=tab] {transductionaccuracy.tex};
\addlegendentry{{\scriptsize Sentence Transduction}};

\end{axis}
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:

